Clustered Planarity = Flat Clustered Planarity

The complexity of deciding whether a clustered graph admits a clustered planar drawing is a long-standing open problem in the graph drawing research area. Several research efforts focus on a restricted version of this problem where the hierarchy of the clusters is "flat", i.e., no cluster different from the root contains other clusters. We prove that this restricted problem, that we call Flat Clustered Planarity, retains the same complexity of the general Clustered Planarity problem, where the clusters are allowed to form arbitrary hierarchies. We strengthen this result by showing that Flat Clustered Planarity is polynomial-time equivalent to Independent Flat Clustered Planarity, where each cluster induces an independent set. We discuss the consequences of these results.

==> makefile <==
finalname = main

included_latex_sources = 
compiler = pdflatex
psfiles = \


$(finalname): $(included_latex_sources) $(psfiles) $(finalname).tex
	$(compiler) $(finalname).tex

%.ps: %.fig
	fig2dev -Leps $< $@

%.ps: %.gif
	convert $< $@

%.ps: %.bmp
	convert $< $@

%.ps: %.jpg
	convert $< $@

startup:
	xemacs $(finalname).tex &
	xdvi $(finalname) &
	xfig -bg white -fg black &

clean:
	rm -f $(psfiles)
	rm -f $(finalname).ps
	rm -f tmp-data/*.avg
	rm -f tmp-data/*.txt
	rm -f src-data/*.tmp
	rm -f *~
	rm -f *.bak
	rm -f figures/*.bak
	rm -f *.toc
	rm -f *.aux
	rm -f *.blg
	rm -f *.dvi
	rm -f *.log
	rm -f *.bbl 
	rm -f *.idx 
	rm -f *.out 
	rm -f $(finalname).pdf
	rm -f *.thm
	rm -f *synctex
	rm -f *synctex.gz
	rm -f *.sav
	rm -f *.vtc
	rm -f *.fdb_latexmk
	rm -f *.fls

bib: 
	$(compiler) $(finalname).tex
	bibtex $(finalname)
	$(compiler) $(finalname).tex
	$(compiler) $(finalname).tex



ps: $(finalname)
	dvips -t a4 $(finalname).dvi -o # -pp 6 -t a4

#	dvips -t letter $(finalname).dvi -o

pdf: 
	$(compiler) $(finalname).tex

level: 
	$(compiler) mainLevel.tex
	
clique: 
	$(compiler) mainClique.tex	
	
print: ps
	lpr -Ppolaris -h $(finalname).ps


